Optimizing Build Orientation for Support Removal using Multi-Axis Machining

Parts fabricated by additive manufacturing (AM) are often fabricated first as a near-net shape, a combination of intended nominal geometry and sacrificial support structures, which need to be removed in a subsequent post-processing stage using subtractive manufacturing (SM). In this paper, we present a framework for optimizing the build orientation with respect to removability of support structures. In particular, given a general multi-axis machining setup and sampled build orientations, we define a Pareto-optimality criterion based on the total support volume and the "secluded" support volume defined as the support volume that is not accessible by a given set of machining tools. Since total support volume mainly depends on the build orientation and the secluded volume is dictated by the machining setup, in many cases the two objectives are competing and their trade-off needs to be taken into account. The accessibility analysis relies on the inaccessibility measure field (IMF), which is a continuous field in the Euclidean space that quantifies the inaccessibility of each point given a collection of tools and fixturing devices. The value of IMF at each point indicates the minimum possible volumetric collision between objects in relative motion including the part, fixtures, and the tools, over all possible tool orientations and sharp points on the tool. We also propose an automated support removal planning algorithm based on IMF, where a sequence of actions are provided in terms of the fixturing devices, cutting tools, and tool orientation at each step. In our approach, each step is chosen based on the maximal removable volume to iteratively remove accessible supports. The effectiveness of the proposed approach is demonstrated through benchmark examples in 2D and realistic examples in 3D.

==> results.tex <==
\section{Results} \label{sec_results}

\begin{figure} [ht!]
	\begin{subfigure}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_fixture1.png}
		\caption{Fixture 1.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_fixture2.png}
		\caption{Fixture 2.}
	\end{subfigure}%
	
	\begin{subfigure}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_fixture3.png}
		\caption{Fixture 3.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_fixture4.png}
		\caption{Fixture 4.}
	\end{subfigure}%
	\caption{Four fixturing devices.} \label{fig_fixtures}
\end{figure}

\begin{figure} [ht!]
	\begin{subfigure}[t]{\linewidth}
		\centering
		\includegraphics[width=0.5\linewidth]{fig/fig_3tools_2D.png}
		\caption{3 different machining tools.}
	\end{subfigure}%

	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_tool1_dirs.png}
		\caption{Tool 1.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_tool2_dirs.png}
		\caption{Tool 2.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig_tool3_dirs.png}
		\caption{Tool 3.}
	\end{subfigure}%
	\caption{Three machining tools and their corresponding orientations.} \label{fig_tools}
\end{figure}

\subsection{Optimizing Build Orientation }

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.75\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_sampledValues100_wt0.png}
		\caption{Sampled orientations and values.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.25\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_SO3_wt0.png}
		\caption{SO3.}
	\end{subfigure}%
	\caption{Sampled orientations and support volumes for $w = 0$.} \label{fig_SO3_wt0}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt1_wt0.png}
		\caption{$\overrightarrow{b} = (0,0,1)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt2_wt0.png}
		\caption{$\overrightarrow{b} = (-0.58,-0.81,-0.05)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt3_wt0.png}
		\caption{$\overrightarrow{b} = (-0.76,0.42,-0.48)$.}
	\end{subfigure}%

	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt4_wt0.png}
		\caption{$\overrightarrow{b} = (0.01,0.14,0.99)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
	\centering
	\includegraphics[width=0.95\linewidth]{fig/fig_opt5_wt0.png}
	\caption{$\overrightarrow{b} = (0,1,0)$.}
\end{subfigure}%
	\caption{5 Pareto-optimal directions with $w = 0$.} \label{fig_nearnets_wt0}
\end{figure*}


\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.75\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_sampledValues100_wt25.png}
		\caption{Sampled orientations and values.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.25\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_SO3_wt25.png}
		\caption{SO3.}
	\end{subfigure}%
	\caption{Sampled orientations and support volumes for $w = 0.25$.} \label{fig_SO3_wt25}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt1_wt25.png}
		\caption{$\overrightarrow{b} = (0,0,1)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt2_wt25.png}
		\caption{$\overrightarrow{b} = (-0.89,-0.31,-0.32)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{fig/fig_opt3_wt25.png}
		\caption{$\overrightarrow{b} = (-0.15,0.38,0.91)$.}
	\end{subfigure}%
	
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt4_wt25.png}
		\caption{$\overrightarrow{b} = (-0.86,0.22,-0.45)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt5_wt25.png}
		\caption{$\overrightarrow{b} = (-0.76,0.42,-0.49)$.}
	\end{subfigure}%
	\caption{5 Pareto-optimal directions with $w = 0.25$.} \label{fig_nearnets_wt25}
\end{figure*}


\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.75\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_sampledValues100_wt50.png}
		\caption{Sampled orientations and values.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.25\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_SO3_wt50.png}
		\caption{SO3.}
	\end{subfigure}%
	\caption{Sampled orientations and support volumes for $w = 0.50$.} \label{fig_SO3_wt50}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt1_wt50.png}
		\caption{$\overrightarrow{b} = (-0.15,0.38,0.91)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt2_wt50.png}
		\caption{$\overrightarrow{b} = (-0.89,-0.31,-0.32)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{fig/fig_opt3_wt50.png}
		\caption{$\overrightarrow{b} = (-0.86,0.22,-0.45)$.}
	\end{subfigure}%
	
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt4_wt50.png}
		\caption{$\overrightarrow{b} = (0.06,0.95,-0.29)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt5_wt50.png}
		\caption{$\overrightarrow{b} = (-0.97,-0.13,-0.21)$.}
	\end{subfigure}%
	\caption{5 Pareto-optimal directions with $w = 0.50$.} \label{fig_nearnets_wt50}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.75\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_sampledValues100_wt75.png}
		\caption{Sampled orientations and values.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.25\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_SO3_wt75.png}
		\caption{SO3.}
	\end{subfigure}%
	\caption{Sampled orientations and support volumes for $w = 0.75$.} \label{fig_SO3_wt75}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt1_wt75.png}
		\caption{$\overrightarrow{b} = (-0.86,0.22,-0.45)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt2_wt75.png}
		\caption{$\overrightarrow{b} = (-0.15,0.39,0.91)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{fig/fig_opt3_wt75.png}
		\caption{$\overrightarrow{b} = (-0.89,-0.31,-0.32)$.}
	\end{subfigure}%
	
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt4_wt75.png}
		\caption{$\overrightarrow{b} = (0.06,0.95,-0.29)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt5_wt75.png}
		\caption{$\overrightarrow{b} = (-0.10,0.43,0.89)$.}
	\end{subfigure}%
	\caption{5 Pareto-optimal directions with $w = 0.75$.} \label{fig_nearnets_wt75}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.75\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_sampledValues100_wt100.png}
		\caption{Sampled orientations and values.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.25\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{fig/fig_SO3_wt100.png}
		\caption{SO3.}
	\end{subfigure}%
	\caption{Sampled orientations and support volumes for $w = 1.0$.} \label{fig_SO3_wt100}
\end{figure*}

\begin{figure*} [ht!]
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt1_wt100.png}
		\caption{$\overrightarrow{b} = (-0.86,0.22,-0.45)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt2_wt100.png}
		\caption{$\overrightarrow{b} = (-0.15,0.39,0.91)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{fig/fig_opt3_wt100.png}
		\caption{$\overrightarrow{b} = (0.06,0.95,-0.29)$.}
	\end{subfigure}%
	
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt4_wt100.png}
		\caption{$\overrightarrow{b} = (-0.89,-0.31,-0.32)$.}
	\end{subfigure}%
	\begin{subfigure}[t]{0.33\linewidth}
		\centering
		\includegraphics[width=0.95\linewidth]{fig/fig_opt5_wt100.png}
		\caption{$\overrightarrow{b} = (-0.95,-0.29,0.05)$.}
	\end{subfigure}%
	\caption{5 Pareto-optimal directions with $w =1.0$.} \label{fig_nearnets_wt100}
\end{figure*}


\subsection{Support Removal Planning}

\begin{figure*} [ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/plan_wt0_opt1.png}
	\caption{8-step support removal plan for optimal orientation with $w = 0$.} \label{fig_plan_wt0_opt1}
\end{figure*}

\begin{figure*} [ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/plan_wt50_opt1.png}
	\caption{10-step support removal plan for optimal orientation with $w = 0.5$.} \label{fig_plan_wt50_opt1}
\end{figure*}

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.9\linewidth]{fig/plan_wt75_opt1.png}
	\caption{8-step support removal plan for optimal orientation with $w = 0.75$.} \label{fig_plan_wt75_opt1}
\end{figure*}
